Group Spike and Slab Variational Bayes

We introduce Group Spike-and-slab Variational Bayes (GSVB), a scalable method for group sparse regression. A fast co-ordinate ascent variational inference (CAVI) algorithm is developed for several common model families including Gaussian, Binomial and Poisson. Theoretical guarantees for our proposed approach are provided by deriving contraction rates for the variational posterior in grouped linear regression. Through extensive numerical studies, we demonstrate that GSVB provides state-of-the-art performance, offering a computationally inexpensive substitute to MCMC, whilst performing comparably or better than existing MAP methods. Additionally, we analyze three real world datasets wherein we highlight the practical utility of our method, demonstrating that GSVB provides parsimonious models with excellent predictive performance, variable selection and uncertainty quantification.

==> settings.tex <==
\RequirePackage{amsthm,amsmath,amsfonts,amssymb}
% \RequirePackage[numbers]{natbib}
\RequirePackage[authoryear]{natbib}%% uncomment this for author-year citations
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,backref=page,backref=page]{hyperref}
\RequirePackage{graphicx}


\usepackage[noend]{algpseudocode}
\usepackage{algorithm}
% \usepackage{amsthm}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% \usepackage{amssymb}
% \usepackage[round]{natbib}
%\usepackage{natbib}
\usepackage{multirow}
\usepackage{stfloats}
\usepackage{float}
% \usepackage{graphicx}
\usepackage{xcolor}
% \usepackage{geometry}
\usepackage{url}
\usepackage{caption}
\usepackage{enumerate}
\usepackage{subcaption}
% \usepackage[
%   bookmarks=false,
%   pdfpagelabels=false,
%   hyperfootnotes=false,
%   hyperindex=false,
%   pageanchor=false,
%   colorlinks,
%   citecolor=blue
% ]{hyperref}
\usepackage{cleveref}
\usepackage{tikz}
% \usepackage{tabularx}
\usepackage{booktabs}
\usepackage{pifont}
% \usepackage[notref, notcite]{showkeys}

\graphicspath{{../figures/}}
% \linespread{1.5}
% \bibliographystyle{abbrvnat}
% \bibliographystyle{plainnat}
\bibliographystyle{chicago}
\newcommand\NoDo{\renewcommand\algorithmicdo{}}     % remove "do" from algs
% \setlength{\parindent}{0em}
% \setlength{\parskip}{.5em}




% note:
% - plot the distirbution of the gelman rubin diagnostics : across the runs
% - for each variable you can also present the gelamn rubin diag
% - each of the variables vs univariate gelman rubin for the runs
